RedApt: An Adaptor for wav2vec 2 Encoding \\ Faster and Smaller Speech Translation without Quality Compromise

Pre-trained speech Transformers in speech translation (ST) have facilitated state-of-the-art (SotA) results; yet, using such encoders is computationally expensive. To improve this, we present a novel Reducer Adaptor block, RedApt, that could be seamlessly integrated within any Transformer-based speech encoding architecture. Integrating the pretrained wav2vec 2 speech encoder with RedAptbrings 41% speedup, 33% memory reduction with 24% fewer FLOPs at inference. To our positive surprise, our ST model with RedApt outperforms the SotA architecture by an average of 0.68 BLEU score on 8 language pairs from Must-C.

==> algorithms/alg-dp.tex <==

\newcommand{\vy}{\pmb{y}}
\newcommand{\vx}{\pmb{x}}
\newcommand{\vX}{\pmb{X}}
\newcommand{\vY}{\pmb{Y}}


\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[!t]
\caption{Constrained segmentation}
\begin{algorithmic}[1]
\REQUIRE{$\vY$: List of unsegmented target utterances, $N:$ Length of target sequence, $\vX:$ List of segmented source, $K:$ Number of source segments, $d$: A distance similarity metric.}
\ENSURE{$T$: The DP table with optimal scores}
\STATE // initialisation
\FOR{$i = 1 ... {N}$}
\STATE $T_{1,i} = d(\vX_1,\vY_{1:i})$
\ENDFOR
\STATE // Filling out $T$ based on the DP relation
\FOR{$k = 2 ... K$}
\FOR{$i = k ... N$}
\STATE $T_{k,i} = \max\limits_{k \le j \le i} \left[T_{k-1,j-1} + d(\vX_k, \vY_{j:i})\right]$ 
\ENDFOR 
\ENDFOR
\RETURN $T$
\end{algorithmic}
\label{alg:npi}
\end{algorithm}

% \begin{algorithm}[t]
% \caption{Constrained segmentation}
% \begin{algorithmic}[1]
% \REQUIRE{$\vY$: List of segmented target utterances, $K:$ number of target segments, $\vx:$ Unsegmented source, $N:$ Length of source sequence}
% \ENSURE{$T$: The DP table with optimal  scores}
% \STATE // initialisation
% \FOR{$i = 1 ... {N}$}
% \STATE $T[1,i] = simScore(\vY[1],\vx_{1:i})$
% \ENDFOR
% \STATE // Filling out $T$ based on the DP relation
% \FOR{$k = 2 ... K$}
% \FOR{$i = k ... N$}
% \FOR{$j = k ... i-1$}
% \STATE $T[k,i] \leftarrow T[k-1,j] +$ 
% \STATE \hspace{15mm} $simScore(\vY[k],\vx_{(j+1):i})$
% \ENDFOR 
% \ENDFOR 
% \ENDFOR
% \RETURN $T$
% \end{algorithmic}
% \label{alg:npi}
% \end{algorithm}

==> figures/figure-ngram.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
    method & adapt & seq2seq & HPBMT(unsup) & PBMT & HPBMT\\
1-gram & 20.71 & 15.95 & 21.83 & 19.59 & 19.52\\
2-gram & 11.14 & 10.48 & 11.34 & 12.13 & 12.16 \\
3-gram & 06.05 & 06.16 & 06.01 & 07.19 & 07.64 \\
4-gram & 03.16 & 03.42 & 03.24 & 04.25 & 04.40 \\
    }\interngram
 

\begin{figure}[!t]
\centering 
  \begin{tikzpicture}[thick,scale=0.73, every node/.style={scale=0.73}]
      \begin{axis}[
            ybar, axis on top,
            title style={at={(0.5,0.97)},anchor=north,yshift=-0.1, draw=gray},
            %title={DE-EN},
            height=7cm, 
            width=8cm,
            bar width=0.17cm,
            ymajorgrids, tick align=inside,
            major grid style=dashed,
            % major grid style={draw=white},
            enlarge y limits={value=.1,upper},
            ymin=0, ymax=25,
            % axis x line*=bottom,
            % axis y line*=right,
            % y axis line style={opacity=0},
            % tickwidth=0pt,
            x tick style={draw=none},
            enlarge x limits=0.15,
            legend style={
                at={(0.5,-0.2)},
                anchor=north,
                legend columns=-1,
                /tikz/every even column/.append style={column sep=0.5cm}
            },
            ylabel={Percentage (\%)},
            ylabel near ticks,
            symbolic x coords={
               1-gram, 2-gram, 3-gram, 4-gram},
           xtick=data,
        ]
        \legend{adapt, seq2seq, HPBMT(unsup), PBMT, HPBMT}
        \addplot[fill=blue!60] table[x=method,y=adapt]{\interngram};
        \addplot[fill=green!60] table[x=method,y=seq2seq]{\interngram};
        \addplot[fill=cyan!60] table[x=method,y=HPBMT(unsup)]{\interngram};
        \addplot[fill=red!60] table[x=method,y=PBMT]{\interngram};
        \addplot[fill=yellow!60] table[x=method,y=HPBMT]{\interngram};
        
      \end{axis}
      \end{tikzpicture}

% \vspace{-3mm}
%}
\caption{Percentage of introduced correct n-grams.}
\label{fig:ngram}
\end{figure}

==> tables/baseline_vs_adaptation.tex <==
\begin{comment}


\begin{table}
\centering
\small
  \scalebox{0.7}
  {
  \begin{tabular}{lccccccccc}
    \toprule
      &\multicolumn{3}{c}{Translation} & \multicolumn{3}{c}{Interpretation(ASR)} & \multicolumn{3}{c}{Interpretation}   \\
    Model  & AP & AL& BLEU & AP & AL& BLEU & AP & AL& BLEU \\
    \midrule
    \addlinespace[0.3em]
    \textit{Europarl} \\
    pre-train wait-k on \textit{<Source, Translation>}  & 0.61 & 2.84 & 22.78$^*$& 0.61 & 2.84 & 11.47$^*$ & 0.61 & 2.84& 12.34$^*$  \\
    %\hspace{2mm} fine-tune on \textit{<source, long\_noised>}  & 0.61&2.93&23.24 & 11.53(0.06)\\
    \hspace{2mm} fine-tune on \textit{<Source-BT, Raw-Inter\footnote{We dropped "Complete" here for the sake of clarity.}>}  & \underline{0.61}& \underline{2.76} &20.71& \underline{0.61}& \underline{2.76}  &12.05 & \underline{0.61}& \underline{2.76} & 12.69 \\
    \hline
    \textit{T2I-Europarl} \\
    train wait-k on \textit{<Source, Pseudo-I>} \\ % \footnote{Pseudo-I were produced by T2I models}
    \hspace{2mm} Seq2seq (unsupervised) &0.66 &4.45 & 10.42 &0.66 &4.45  &7.79 &0.66 &4.45 & 10.33 \\
    \hspace{2mm} HPBMT (unsupervised) & 0.61& 2.92&18.80 & 0.61& 2.92 & 13.53 & 0.61& 2.92 & 13.21  \\
    \hspace{2mm} PBMT (supervised) & 0.61 & 2.93 & 17.34 & 0.61 & 2.93 & 13.87 & 0.61 & 2.93 & 13.56  \\
    \hspace{2mm} HPBMT (supervised) &0.62 &3.00 & 18.55 &0.62 &3.00 & \textbf{14.26} &0.62 &3.00 & \textbf{13.60} \\
    \bottomrule
  \end{tabular}
  }
  \caption{Evaluation on human annotated Translation Test, Interpretation Test(ASR) and Interpretation Test. $^*$: performance gap in evaluation. \underline{Underlined}: lowest delay across systems. \textbf{Bold}: Best BLEU on Interpretation Test.
  }
  \label{tab:focus} 
  \vspace{-2.5mm}
\end{table}
\end{comment}

\begin{comment}
\begin{table*}
\centering
\small
  \scalebox{0.6}
  {
  \begin{tabular}{lccccc}
    \toprule
      & & \multicolumn{4}{c}{BLEU}  \\
    Model  & AP & AL& Translation & Interpretation(ASR) & Interpretation \\
    \midrule
    \addlinespace[0.3em]
    \textit{Europarl} \\
    pre-train on \textit{<Source, Translation>}  & 0.61 & 2.84 & 22.78 & 11.47 & 12.34  \\
    %\hspace{2mm} fine-tune on \textit{<source, long\_noised>}  & 0.61&2.93&23.24 & 11.53(0.06)\\
    \hspace{2mm} fine-tune on \textit{<Source\_BT, Raw-Inter>}  & \textbf{0.61}& \textbf{2.76} &20.71  &12.05 & 12.69 \\
    \hline
    \textit{T2I-Europarl} \\
    train on \textit{<Source, Pseudo-I>} \\ %\footnote{Pseudo-I were produced by T2I models}
    \hspace{2mm} Seq2seq (unsupervised) &0.66 &4.45 & 10.42  &7.79 & 10.33 \\
    \hspace{2mm} HPBMT (unsupervised) & 0.61& 2.92&18.80 & 13.53 & 13.21  \\
    \hspace{2mm} PBMT (supervised) & 0.61 & 2.93 & 17.34  & 13.87 & 13.56  \\
    \hspace{2mm} HPBMT (supervised) &0.62 &3.00 & 18.55 & \textbf{14.26} & \textbf{13.60} \\
    \bottomrule
  \end{tabular}
  }
  \caption{Evaluation on human annotated Translation Test and Interpretation Test. $^*$: inside the parentheses are the changes in BLEU on the clean Interpretation Test. 
  }
  \label{tab:focus} 
  \vspace{-2.5mm}
\end{table*}
\end{comment}


\begin{comment}


\begin{table}[t]
\centering
\small
  \scalebox{0.65}
  {
  \begin{tabular}{lcc}
    \toprule
    Model  & Interpretation & Interpretation(Clean)  \\
    \midrule
    \addlinespace[0.3em]
    Pre-train on Europarl & 11.47 & 0.89 $\uparrow$ \\
    \hspace{2mm} Fine-tune on raw\_inter & 12.05 & 0.64 $\uparrow$ \\
    Train on Europarl\_T2I  \\
    \hspace{2mm} T2I\textbackslash HPBMT (unsupervised) &13.53&0.30$\downarrow$\\
    \hspace{2mm} T2I\textbackslash PBMT & 13.87 & 0.60 $\downarrow$ \\ 
    \hspace{2mm} T2I\textbackslash HPBMT &14.26&0.60 $\downarrow$\\
    \bottomrule
  \end{tabular}
  }
  \caption{Measure translation quality in BLEU on Interpretation Test with ASR errors and clean Interpretation Test. 
  %$^*$: indices refer to data configurations for training SMT. \dag: same test set as PBMT (1). 
  %Use of EPTIC showcased the effects of using clean transcript.
  }
  \label{tab:two_versions} 
  \vspace{-2.5mm}
\end{table}
\end{comment}

% \begin{table}[t]
% \centering
% \small
%   \scalebox{0.6}
%   {
%   \begin{tabular}{lcccc}
%     \toprule
%       & & \multicolumn{3}{c}{BLEU}  \\
%     Model  & AP & AL& Translation & Interpretation  \\
%     \midrule
%     \addlinespace[0.3em]
%     \textit{Europarl} \\
%     pre-train on \textit{<source, translation>}  & 0.61 & 2.84 & 22.78 & 11.47   \\
%     \hline

%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Evaluation on human annotated Translation Test and Interpretation Test for German, French, Polish and Italian. 
%   }
%   \label{tab:focus} 
%   \vspace{-2.5mm}
% \end{table}

% \begin{table}[t]
% \centering
% \small
%   \scalebox{0.6}
%   {
%   \begin{tabular}{lccccccccc}
%     \toprule
%     &  \multicolumn{3}{c}{Translation Test} & \multicolumn{3}{c}{Interpretation Test} & \multicolumn{3}{c}{Interpretation Test(Clean)} \\
%     Model  & AP & AL& Bleu & AP & AL& Bleu& AP & AL& Bleu \\
%     \midrule
%     \addlinespace[0.3em]
%     Europarl \\
%     \hspace{2mm} wait-k  & 0.61 & 2.84 & 22.78 & 0.61 & 2.84 & 11.47 & 0.61& 2.84&12.34  \\
%   % \hspace{2mm} + Long-noised & 0.61&2.93 &23.24 & 0.61&2.93 & 11.53& 0.61&2.93 &12.42 \\
%     \hspace{2mm} + Mono-inter (BT)  & \textbf{0.61}& \textbf{2.76} &20.71 &\textbf{0.61}& \textbf{2.76} &12.05 &\textbf{0.61}& \textbf{2.76} &12.69\\
%     \hline
%     Europarl\_T2I   \\
%     \hspace{2mm} Seq2seq &0.66 &4.45 & 10.42&0.66 &4.45  &7.79 &0.66 &4.45 & 10.33\\
%     \hline
%     Europarl\_T2I   \\
%     \hspace{2mm} PBMT (1)$^*$ & 0.61 & 2.93 & 17.34  & 0.61 & 2.93 & 13.87 &0.61 &2.93 & 13.56 \\
%     \hspace{2mm} PBMT (2) & 0.62 & 2.95&18.83 &0.62 &2.95 &14.22 &0.62 &2.95 & \textbf{14.02} \\
%     \hspace{5mm} + EPTIC (BT) \\
%     \hspace{2mm} HPBMT (1) &0.62 &3.00 & 18.55 &0.62 &3.00 & \textbf{14.26} &0.62 &3.00&13.60  \\%& 0.60 & 2.82 & 16.50 & 0.60 & 2.82 & 20.98 & 0.62 & 3.00 & 18.51 & 0.62 & 3.00 & 14.32 & & & \\
%     \hspace{2mm} HPBMT (2)  &0.62 &2.96 &19.47 & 0.62&2.96 &13.84 &0.62 &2.96 &13.53\\
%     \hspace{2mm}\textit{Unsupervised} \\
%     % \hspace{2mm} PBMT1 &0.60 &2.67 &16.88 &0.61 &2.82 &20.51 & 0.61 & 2.82&18.38 &0.61 &2.82 &12.80 \\
%     %\hspace{2mm} PBMT1 & 0.60& 2.69&17.21 &0.60 &2.69 &21.02 &0.61 &2.88 &18.62$^*$ &0.61 &2.88 &13.02$^*$ \\
%     % \hspace{2mm} HPBMT1  \\
%     %\hspace{2mm} HPBMT (1) & 0.60& 2.78&14.81 &0.60 &2.78 &19.73 & 0.62 &2.97 & 16.82& 0.62&2.97 &13.22 &0.62 &2.96 &13.01 \\
%     \hspace{2mm} HPBMT (2) & 0.61& 2.92&18.80 &0.61 &2.92 & 13.53 &0.61 &2.92 & 13.21 \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Evaluation on Europarl, Europarl\_T2I, our human annotated Translation Test and Interpretation Test . $^*$: indices refer to data configurations for training SMT. \dag: same test set as PBMT (1). Use of EPTIC showcased the effects of using clean transcript.}
%   \label{tab:focus} 
%   \vspace{-2.5mm}
% \end{table}

% \begin{table*}[t]
% \centering
% \small
%   \scalebox{0.83}
%   {
%   \begin{tabular}{lccccccccccccccc}
%     \toprule
%     &  \multicolumn{3}{c}{Europarl Test}  & \multicolumn{3}{c}{Europarl\_T2I Test} & \multicolumn{3}{c}{Translation Test} & \multicolumn{3}{c}{Interpretation Test} & \multicolumn{3}{c}{Interpretation Test(Clean)} \\
%     Model & AP & AL & Bleu &AP & AL & Bleu  & AP & AL& Bleu & AP & AL& Bleu& AP & AL& Bleu \\
%     \midrule
%     \addlinespace[0.3em]
%     Europarl \\
%     \hspace{2mm} wait-k &0.62 & 3.40 & 23.59 & 0.62 &3.40  &18.18\dag  & 0.61 & 2.84 & 22.78 & 0.61 & 2.84 & 11.47 & 0.61& 2.84&12.34  \\
%     \hspace{2mm} + Long-noised &0.60 &2.70 & 22.07&0.60 &2.70 & 17.34\dag & 0.61&2.93 &23.24 & 0.61&2.93 & 11.53& 0.61&2.93 &12.42 \\
%     \hspace{2mm} + Mono-inter (BT) &\textbf{0.59} &\textbf{2.58} &19.64 &\textbf{0.59} &\textbf{2.58} & 16.12\dag & \textbf{0.61}& \textbf{2.76} &20.71 &\textbf{0.61}& \textbf{2.76} &12.05 &\textbf{0.61}& \textbf{2.76} &12.69\\
%     \hline
%     Europarl\_T2I   \\
%     \hspace{2mm} Seq2seq & 0.64 & 4.3&10.56 & 0.64 & 4.3 &17.55 &0.66 &4.45 & 10.42&0.66 &4.45  &7.79 &0.66 &4.45 & 10.33\\
%     \hline
%     Europarl\_T2I   \\
%     \hspace{2mm} PBMT (1)$^*$ & 0.60 & 2.77 & 16.22 &0.60  & 2.77 & 20.06 & 0.61 & 2.93 & 17.34  & 0.61 & 2.93 & 13.87 &0.61 &2.93 & 13.56 \\
%     \hspace{2mm} PBMT (2) & 0.60 & 2.78 & 17.47& 0.60 & 2.78 & 21.10 & 0.62 & 2.95&18.83 &0.62 &2.95 &14.22 &0.62 &2.95 & \textbf{14.02} \\
%     \hspace{5mm} + EPTIC (BT) \\
%     \hspace{2mm} HPBMT (1)  &0.60 & 2.82&16.47 &0.60 & 2.82& 20.98&0.62 &3.00 & 18.55 &0.62 &3.00 & \textbf{14.26} &0.62 &3.00&13.60  \\%& 0.60 & 2.82 & 16.50 & 0.60 & 2.82 & 20.98 & 0.62 & 3.00 & 18.51 & 0.62 & 3.00 & 14.32 & & & \\
%     \hspace{2mm} HPBMT (2)  &0.60  &2.79 &17.87 & 0.60& 2.79 &22.58 &0.62 &2.96 &19.47 & 0.62&2.96 &13.84 &0.62 &2.96 &13.53\\
%     \hspace{2mm}\textit{Unsupervised} \\
%     % \hspace{2mm} PBMT1 &0.60 &2.67 &16.88 &0.61 &2.82 &20.51 & 0.61 & 2.82&18.38 &0.61 &2.82 &12.80 \\
%     %\hspace{2mm} PBMT1 & 0.60& 2.69&17.21 &0.60 &2.69 &21.02 &0.61 &2.88 &18.62$^*$ &0.61 &2.88 &13.02$^*$ \\
%     % \hspace{2mm} HPBMT1  \\
%     %\hspace{2mm} HPBMT (1) & 0.60& 2.78&14.81 &0.60 &2.78 &19.73 & 0.62 &2.97 & 16.82& 0.62&2.97 &13.22 &0.62 &2.96 &13.01 \\
%     \hspace{2mm} HPBMT (2) & 0.60 &2.73 &17.44 & 0.60 & 2.73 & 22.39& 0.61& 2.92&18.80 &0.61 &2.92 & 13.53 &0.61 &2.92 & 13.21 \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Evaluation on Europarl, Europarl\_T2I, our human annotated Translation Test and Interpretation Test . $^*$: indices refer to data configurations for training SMT. \dag: same test set as PBMT (1). Use of EPTIC showcased the effects of using clean transcript.}
%   \label{tab:focus} 
%   \vspace{-2.5mm}
% \end{table*}


% \begin{table*}
% \centering
% \small
%   \scalebox{0.85}
%   {
%   \begin{tabular}{l|ccc|ccc|ccc|ccc}
%     \toprule
%     &  \multicolumn{3}{c}{Europarl Test}  & \multicolumn{3}{c}{Europarl\_T2I Test} & \multicolumn{3}{c}{Translation Test} & \multicolumn{3}{c}{Interpretation Test} \\
%     Model & AP & AL & Bleu &AP & AL & Bleu  & AP & AL& Bleu & AP & AL& Bleu\\
%     \midrule
%     \addlinespace[0.3em]
%     Wait-3 &  \\
%     - Europarl &0.62 & 3.4 & 23.59 & 0.65 &3.80  &18.18  & 0.64 & 3.63 & 24.42 & 0.64 & 3.63 & 11.90   \\
%     \hspace{2mm} + D2 &0.59 &2.58 &19.64 & 0.60&2.58&16.12 & 0.61&2.77 &20.75 &0.61 &2.77 &11.94 \\
%     - Europarl\_T2I   \\
%     \hspace{2mm} - PBMT1 &  &  &  &0.60  & 2.77 & 20.06 & 0.61 & 2.93 & 17.34  & 0.61 & 2.93 & 13.87 \\
%     \hspace{2mm} - PBMT2 & 0.60 & 2.78 & 17.47& 0.60 & 2.78 & 21.10 & 0.62 & 2.96 & 18.81 & 0.62 & 2.96 & \textbf{14.40} \\
%     \hspace{2mm} - Hier & 0.60 & 2.82 & 16.50 & 0.60 & 2.82 & 20.98 & 0.62 & 3.00 & 18.51 & 0.62 & 3.00 & 14.32  \\
%     \hline
%     \addlinespace[0.3em]
%     Coupled Policy & \\
%     - Europarl &0.65 &3.75 & \textbf{23.09} & 0.65 &3.75  & 18.18 & 0.67 &4.22 &\textbf{23.63} & 0.67 &4.22 &11.39  \\
%       \hspace{2mm} + D2 & 0.63 & 3.07& 20.97 & 0.64&3.07 &17.14 & 0.64&3.13 &20.64   &0.64& 3.13&12.18 \\
%     - Europarl\_T2I   \\
%     \hspace{2mm} - PBMT1 & 0.65 & 3.79  & 16.03 & 0.65 & 3.79 & 19.57 & 0.68 & 4.66  & 16.62 & 0.68 & 4.66 & 12.85 \\
%     \hspace{2mm} - PBMT2 & 0.64 & 3.05 & 16.41 & 0.64 & 3.05 & 19.30 & 0.66 & 3.70 & 17.22 & 0.66 & 3.70 & 12.41 \\
%     \hspace{2mm} - Hier & 0.64 & 3.40 & 16.48 & 0.64 & 3.40 & 20.83 & 0.66 & 3.80 & 17.77 & 0.66 & 3.80 & 12.86  \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Europarl vs Europarl\_T2I. }
%   \label{tab:focus}
% \end{table*}



\iffalse
\begin{table*}
\centering
\small
  \scalebox{0.7}
  {
  \begin{tabular}{l|l|ccc|ccc|ccc|ccc}
    \toprule
   & &  \multicolumn{3}{c}{Europarl Test}  & \multicolumn{3}{c}{Europarl\_T2I Test} & 
    \multicolumn{3}{c}{EPTIC-translation} &
    \multicolumn{3}{c}{EPTIC-interpretation} \\
    & Model & AP & AL & Bleu &AP & AL & Bleu  & AP & AL& Bleu & AP & AL& Bleu\\
    \midrule
    \addlinespace[0.3em]
     & Wait-3   \\
    Fr & - Europarl & 0.58&2.40 &21.24 &0.58 &2.40 &17.41 &0.58 &2.41 &23.60 &0.58  &2.41 &9.28   \\
       & - Europarl\_T2I (hier2) & 0.58&2.49 & 18.44&0.58 &2.49 &22.63 & 0.58&2.49 &22.22 &0.58  &2.49 &9.73  \\
    \midrule
    & Wait-3   \\
    Pl & - Europarl & 0.61& 2.88&25.57 &0.61 &2.88 &20.64 &0.61 &2.99 &23.99 &0.61  &2.99 &13.71 \\
       & - Europarl\_T2I (hier-d3-unsup)&0.61&3.00 &20.71 &0.61 &3.00 &25.48 &0.61 &2.98 &21.36 &0.61  &2.98 &13.05    \\
       & - Europarl\_T2I (hier-real-d3-unsup) & 0.61&2.95 &20.09&0.61&2.95&25.78& 0.61&2.89 &21.01 &0.61&2.89&12.67  \\
       & - Europarl\_T2I (hier-real-d3-sup) & 0.61 &3.03 &21.09&0.61&3.03&25.06& 0.61&2.96 &22.02 &0.61&2.96&13.08  \\
    \midrule
    & Wait-3   \\
    It & - Europarl & 0.59 &2.73 &24.47 &0.59 &2.73 &18.79 &0.56 &2.45 &24.41 & 0.56 &2.45 &10.64 \\
       & - Europarl\_T2I (hier2) & 0.60 &2.81 &19.31 &0.60 &2.81 &24.46 &0.57 &2.51 &20.83 &0.57  &2.51 & 9.49 \\
    \bottomrule
  \end{tabular}
  }
  \caption{Europarl vs Europarl\_T2I for French, Polish, Italian, with hier2. \ehsan{we should mention in the text these evaluation results which highlights the real gap. I will do this tmrw.} }
  \label{tab:eptic}
\end{table*}
\fi

% \begin{table*}
% \centering
% \small
%   \scalebox{0.85}
%   {
%   \begin{tabular}{l|ccc|ccc}
%     \toprule
%     &  \multicolumn{3}{c}{IWSLT}  & \multicolumn{3}{c}{Annotated Test}\\
%     Model & AP & AL  & Bleu  & AP & AL& Bleu\\
%     \midrule
%     \textit{Baseline}\\
%     \addlinespace[0.3em]
%     wait-3 & 0.65 & 2.95 & 21.26 & 0.60 & 2.78 & 7.52 \\
%     Coupled Policy & 0.62 & 2.39  & 21.50 & 0.62 & 2.71  & 7.46 \\
%     \hline
%     \textit{Adaptation} \\
%     \addlinespace[0.3em]
%     wait-3 & 0.64 & 2.94 & 21.41 & 0.60 & 2.74 & 9.30 \\
%     Coupled Policy & 0.63 & 2.37 & 19.80 & 0.63 & 2.76 & 9.68 \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Baseline vs Adaptation models.}
%   \label{tab:focus}
% \end{table*}

==> tables/dataset_statistics.tex <==
\begin{table}[t]
\small
    \centering
    \scalebox{0.8}{
    \begin{tabular}{ l  l l l  }
    \toprule
    Datasets & train & dev & test \\
    \midrule
    % IWSLT &  191,751/887/6,996 \\

    % EUROPARL(fr-en) & \\
    % EUROPARL(pl-en) &  \\
    % EUROPARL(it-en) & \\
    \cmss{Raw-Inter (filtered)} & 217622 (120114) & 1000 & - \\
    %Mono-Inter (filtered) & 120,114/-/- \\
    %Long-Noised & 2,983/300/-  \\
    % D2 & 71,431/500/- \\
    \cmss{Clean-Inter (filtered)} & 10021 (4240) & - & - \\
    %Short-Noised (filtered) & 4,240/-/- \\
    %Translation/Interpretation test & - & - & 1051$^*$ \\
    %Interpretation test & -/-/1,051$^*$ \\
    %Europarl/Europarl\_T2I & 1666904 & 3587 & 5075$^*$ \\
    EPTIC & 1636 & - & - \\
    %Inter-Europarl& 1,666,904/3,587/5,075$^*$\\
    \bottomrule
    \end{tabular}}
    \caption{Dataset statistics. $^*$: Data points that are heavily overlapped with any training data are removed.\ehsan{this table now seems insignificant and we can merge this into text}}
    \label{tab:data}
    \vspace{-2.5mm}
\end{table}

==> tables/full_europarl_annotated.tex <==
\begin{comment}


\begin{table*}
\centering
\small
  \scalebox{0.75}
  {
  \begin{tabular}{l|cccc|cccc|cccc|cccc}
    \toprule
    &  \multicolumn{4}{c}{EUROPARL}  & \multicolumn{4}{c}{Translation Test} & \multicolumn{4}{c}{Translation-suboptimal Test} & \multicolumn{4}{c}{Interpretation Test}\\
    Model & AP & AL & Bleu & Meteor & AP & AL& Bleu & Meteor & AP & AL& Bleu & Meteor & AP & AL& Bleu & Meteor\\
    \midrule
    % \textit{wait-2}\\
    % \addlinespace[0.3em]
    % Europarl  & 0.57& 2.03&20.90 &0.58 &2.19 &22.86 &0.58 &2.19 &11.24  \\
    % D1 + Europarl (PTFT) &0.57 &2.04 &19.91 & 0.59& 2.23&21.12 &0.59 & 2.22& 10.67 \\
    % D2 + Europarl (PTFT)  & 0.57& 1.94& 18.20& 0.58& 2.07& 19.15& 0.58&2.07 &11.30 \\
    % %D3 + Europarl (PTFT) & & & & & & & & & \\
    % D1 + D2 + Europarl (PTFT) &0.57 &1.95 &18.10 & 0.58& 2.11&18.93 & 0.58& 2.11&11.35 \\ 
    % %D1 + D2 + D3 + Europarl (PTFT) & & & & & & & & & \\ 
    % D2  &0.58 &2.13 &8.70 & 0.59& 2.24&10.48 & 0.59&2.24 &9.45 \\
    % D1 + Europarl (MIX) & 0.57& 1.98& 17.00& 0.58& 2.14&18.11 &0.58 & 2.14& 9.52  \\
    % D2 + Europarl (MIX) & 0.57&1.93 & 17.09& 0.58& 2.06&18.32 &0.58 &2.06 &11.08 \\
    % %D3 + Europarl (MIX) & & & & & & & & & \\
    % D1 + D2 + Europarl (MIX) &0.57 &1.90 & 15.69& 0.58&2.06 &16.70 & 0.58& 2.06& 10.62 \\ 
    
    % %D1 + D2 + D3 + Europarl (MIX) & & & & & & & & & \\ 
    % \hline
    \textit{wait-3} \\
    \addlinespace[0.3em]
    Europarl  &0.60 & 2.66&21.52& & 0.61& 2.84&22.82 && & & &&0.61 &2.84 &11.38 & \\
    Europarl-suboptimal \\
    D1 + Europarl (PTFT) &0.60 &2.70 & 22.07&& 0.61&2.93 &23.16& & & & &&0.61 &2.93 &11.52& \\
    D2 + Europarl (PTFT) &0.59 &2.58 &19.64 && 0.61&2.77 &20.75& & & & &&0.61 &2.77 &11.94& \\
    %D3 + Europarl (PTFT) & & & & & & & & & \\
    D1 + D2 + Europarl (PTFT) &0.59 &2.57 &19.38 &&0.61 &2.71 &20.18& & & & & &0.61& 2.71& 11.58 &\\ 
    %D1 + D2 + D3 + Europarl (PTFT) & & & & & & & & & \\ 
    D2  & 0.61& 2.78& 9.39&&0.62 & 2.90&11.07& & & & &&0.62 &2.90 &9.63& \\
    D1 + Europarl (MIX) & 0.59&2.71 &22.29& &0.62 &2.95 &23.21& & & & &&0.61 &2.95 &11.79& \\
    D2 + Europarl (MIX) & 0.59& 2.56&18.36 &&0.61 &2.72 &19.72 && & & &&0.61 &2.72 &11.49& \\
    %D3 + Europarl (MIX) & & & & & & & & & \\
    D1 + D2 + Europarl (MIX) &0.59 &2.59 &17.61& &0.61&2.78 &18.89 && & & &&0.61 &2.78 & 11.10& \\ 
    %D1 + D2 + D3 + Europarl (MIX) & & & & & & & & & \\ 
    \hline
    \textit{wait-4} \\
    Europarl  & 0.62& 3.40& \textbf{23.59} &&0.64 &3.63 & \textbf{24.42}& & & & &&0.64 &3.63 &11.90&  \\
    Europarl-suboptimal \\
    D1 + Europarl (PTFT) & 0.62& 3.46&23.05 &&0.64 &3.66 &23.40& & & & & &0.64& 3.66&11.65& \\
    D2 + Europarl (PTFT) &0.62 &3.30 &20.85& &0.64 &3.51 & 22.06 && & & & &0.64& 3.51& \textbf{12.79}& \\
    %D3 + Europarl (PTFT) & & & & & & & & & \\
    D1 + D2 + Europarl (PTFT) & 0.62& 3.32& 21.02&&0.64 &3.52 &21.66 && & & & &0.64& 3.52&12.47& \\ 
    %D1 + D2 + D3 + Europarl (PTFT) & & & & & & & & & \\ 
    D2  & 0.63& 3.49&10.00 &&0.65 &3.72 &11.68 && & & &&0.65 &3.72 &10.27 &\\
    D1 + Europarl (MIX) & 0.62 &3.27 &19.32 &&0.64 &3.49 &20.30& & & & &&0.64 &3.49 &10.34& \\
    D2 + Europarl (MIX) & 0.62& 3.29& 19.00&&0.64 &3.51 &19.62 && & & &&0.64 &3.51 &11.80& \\
    %D3 + Europarl (MIX) & & & & & & & & & \\
    D1 + D2 + Europarl (MIX) & 0.62& 3.21&18.22& &0.64 &3.39 &18.70 && & & &&0.64 &3.39 &11.31 &\\ 
    %D1 + D2 + D3 + Europarl (MIX) & & & & & & & & & \\ 
    \hline
    \textit{Coupled Policy}\\
    \addlinespace[0.3em]
    Europarl  &0.65 &3.75 & \textbf{23.09} &&0.67 &4.22 &\textbf{23.63} && & & &&0.67 &4.22 &11.39&  \\
    Europarl-suboptimal \\
    D1 + Europarl (PTFT) & 0.75 & 5.54 & 18.56 && 0.75& 4.85&19.55& & & & & &0.75 &4.85 &9.76 &\\
    D2 + Europarl (PTFT) & 0.63 & 3.07& 20.97&& 0.64&3.13 &20.64 && & & & &0.64& 3.13&\textbf{12.18}& \\
    %D3 + Europarl (PTFT) & & & & & & & & & \\
    D1 + D2 + Europarl (PTFT)  &0.95 &16.89 &13.59 && 0.95 & 13.70 &14.30 && & & & &0.95 & 13.70 & 8.49 &\\ 
    %D1 + D2 + D3 + Europarl (PTFT) & & & & & & & & & \\ 
    D2  & 0.62& 2.15& 10.60&& 0.64& 2.72& 12.00&& & & && 0.64 &2.72 &10.42 &\\
    D1 + Europarl (MIX) &0.67 & 5.00 &18.31& &0.69 & 5.05& 18.31 & & & & & &0.69&5.05 &9.49 &\\
    D2 + Europarl (MIX) &0.63 &2.69 & 19.02&& 0.66& 3.34& 18.89 && & & & &0.66 & 3.34& 11.26&\\
    %D3 + Europarl (MIX) & & & & & & & & & \\
    D1 + D2 + Europarl (MIX) &0.63 & 2.64& 17.91&& 0.65&3.10 &18.34 &&& & & & 0.64& 3.10& 10.92&\\ 
    %D1 + D2 + D3 + Europarl (MIX) & & & & & & & & & \\ 
    \bottomrule
  \end{tabular}
  }
  \caption{Europarl: Out-of-domain data from EUROPARL. 
  PTFT: Pre-train Fine-tune domain adaptation. MIX: Mixture domain adaptation. \textbf{Bold}: The best results.
  \philip{We need to redo most of the experiment. First: (1) it is better to use EUROPARL original dataset for pretrain. This dataset is more comparable to our dataset. (2) We have to compare translating from $x$ to $y_i$ vs $x$ to $y_o$ and shows that it is better for us to translate from $x$ to $y_i$} }
  %ADV: Adversarial domain adaptation (not the priority for now). BKT: domain adaptation with back-translation.}
  \label{tab:results}
\end{table*}
\end{comment}
% \begin{table*}
% \centering
% \small
%   \scalebox{0.85}
%   {
%   \begin{tabular}{l|ccc|ccc}
%     \toprule
%     &  \multicolumn{3}{c}{IWSLT}  & \multicolumn{3}{c}{Annotated Test}\\
%     Model & AP & AL  & Bleu  & AP & AL& Bleu\\
%     \midrule
%     \textit{wait-2}\\
%     \addlinespace[0.3em]
%     Europarl & 0.61 & 2.26  & 20.00 & 0.58 & 2.14  & 7.31 \\
%     D1 + Europarl (PTFT) & 0.61 & 2.27  & 19.93  & 0.57 & 2.11  & 6.93 \\
%     D2 + Europarl (PTFT) & 0.60 & 2.16  & 19.42  & 0.57 & 1.93  & 7.90 \\
%     D1 + D2 + Europarl (PTFT) & 0.61 & 2.19 & 19.80 & 0.57 & 1.91 & 8.55 \\ 
%     D2 & 0.61 & 2.24 & 5.03  & 0.57 & 1.97 & 5.24 \\
%     D1 + Europarl (MIX) & 0.61 & 2.37 & 18.08 & 0.58 & 2.29 & 5.87 \\
%     D2 + Europarl (MIX) & 0.61 & 2.21 & 17.56 & 0.57  & 1.91 & 7.70 \\
%     D1 + D2 + Europarl (MIX) & 0.62 & 2.66 & 14.64 & 0.58 & 2.36 & 6.28 \\ 
%     \hline
%     \textit{wait-3} \\
%     \addlinespace[0.3em]
%     Europarl & 0.65 & 2.95 & 21.26 & 0.60 & 2.78 & 7.52 \\
%     D1 + Europarl (PTFT) & 0.64 &2.94 & \textbf{22.03} & 0.60 & 2.71& 7.38  \\
%     D2 + Europarl (PTFT) & 0.64 & 2.94 & 21.41 & 0.60 & 2.74 & \textbf{9.30} \\
%     D1 + D2 + Europarl (PTFT) & 0.64 & 2.90 & 20.99 & 0.59 & 2.62 & 9.02 \\ 
%     D2 & 0.64 & 2.85 & 6.04 & 0.60 & 2.54& 6.16\\
%     D1 + Europarl (MIX) & 0.64 & 2.93 & 17.33 & 0.60& 2.80 & 5.95  \\
%     D2 + Europarl (MIX) & 0.64 & 2.93 & 20.10 & 0.60 & 2.59 & 8.70 \\
%     D1 + D2 + Europarl (MIX) & 0.65 & 3.27 & 15.94 & 0.61 & 2.94 & 7.06 \\ 
%     \hline
%     \textit{wait-4} \\
%     Europarl & 0.68 & 3.73 & 23.21 & 0.63 & 3.46 & 7.88  \\
%     D1 + Europarl (PTFT) & 0.68 & 3.75 & 22.52 & 0.63 & 3.42 & 7.63  \\
%     D2 + Europarl (PTFT) & 0.68 & 3.64 & 22.17 & 0.62 & 3.28 & 9.55  \\
%     D1 + D2 + Europarl (PTFT) & 0.68 & 3.65 & 22.11 & 0.62 & 3.25 & 9.20  \\ 
%     D2 & 0.68 & 3.65 & 6.28 & 0.62 & 3.31& 6.52 \\
%     D1 + Europarl (MIX) & 0.68 & 3.75& 18.82& 0.63& 3.57& 6.00  \\
%     D2 + Europarl (MIX) & 0.68 & 3.69 & 21.22 & 0.62 & 3.20 & 9.31 \\
%     D1 + D2 + Europarl (MIX) & 0.68 & 3.79 & 19.29 & 0.62 & 3.32 & 8.44 \\ 
%     \hline
%     \textit{Coupled Policy}\\
%     \addlinespace[0.3em]
%     Europarl & 0.62 & 2.39  & 21.50 & 0.62 & 2.71  & 7.46 \\
%     D1 + Europarl (PTFT) & 0.63 & 2.44  & 21.57 & 0.63 & 2.81  & 7.68 \\
%     D2 + Europarl (PTFT) & 0.63 & 2.45 & \textbf{21.81} & 0.62 & 2.68  & 9.14 \\ 
%     D1 + D2 + Europarl (PTFT) & 0.63 & 2.44 & 20.75 & 0.61 & 2.54 & 9.49 \\
%     D2 & 0.65 & 2.99  & 7.03 & 0.64 & 3.48  & 6.53 \\
%     D1 + Europarl (MIX) & 0.63 & 2.63 & 18.02 & 0.62 & 2.85 & 5.70 \\
%     D2 + Europarl (MIX) & 0.63 & 2.37 & 19.80 & 0.63 & 2.76 & \textbf{9.68} \\
%     D1 + D2 + Europarl (MIX) & 0.62 & 2.42 & 20.04 & 0.61 & 2.66 & 9.10\\ 
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Europarl: Out-of-domain data from IWSLT 2016. 
%   PTFT: Pre-train Fine-tune domain adaptation. MIX: Mixture domain adaptation. \textbf{Bold}: The best results.
%   \philip{We need to redo most of the experiment. First: (1) it is better to use EUROPARL original dataset for pretrain. This dataset is more comparable to our dataset. (2) We have to compare translating from $x$ to $y_i$ vs $x$ to $y_o$ and shows that it is better for us to translate from $x$ to $y_i$}}
%   %ADV: Adversarial domain adaptation (not the priority for now). BKT: domain adaptation with back-translation.}
%   \label{tab:results}
% \end{table*}

==> tables/intro_example.tex <==
% \begin{table}[h]
%     \small
%   \scalebox{0.85}{
%     \begin{tabular}{|p{8cm}|}
%     \hline
%         \textit{\textbf{Source:}} \textcolor{DarkGreen}{Ich werde \ulnum{at\_this\_point}{an diesem Punkt} \ulnum{refrain\_from\_commenting}{darauf verzichten, einen Kommentar} zur  \ulnum{seriousness\_of\_this\_line\_of\_argument}{ Ernsthaftigkeit dieser Argumentationsweise abzugeben}.}  \\
%         \textit{\textbf{Translation:}} \textcolor{violet}{At this point, I will refrain from commenting on the seriousness of this line of argument.}  \\ 
%         \textit{\textbf{Interpretation:}} \textcolor{blue}{I'm not going to comment on that agreement.} \\
%     \hline
%     \end{tabular}}
%     \caption{Example of offline translation and interpretation sentences.}
%     \label{tab:intro_example}
% \end{table}
\begin{table}[t]
    \small
   \scalebox{0.85}{
    \begin{tabular}{|p{8cm}|}
    \hline
        \textit{\textbf{Source:}}
        \textcolor{violet}{\ulnum{I'm}{Ich werde} \ulnum{at\ this\ point}{an diesem Punkt} \ulnum{refrain\ from}{darauf verzichten}, \ulnum{}{einen} \ulnum{to\ comment\ on\ the\
seriousness\ of\ this\ line\ of\ reasoning}{Kommentar zur  Ernsthaftigkeit dieser Argumentationsweise} \ulnum{}{abzugeben}}.  \\
        \textit{\textbf{Offline Translation:}} \textcolor{DarkBlue}{\boldorange{(}At this point,\boldorange{)} I will refrain from commenting on the \redwave{seriousness of this line of argument}.}  \\ 
        \textit{\textbf{Interpretation:}} \textcolor{DarkGreen}{I'm not going to comment on that \redwave{agreement}.} \\
    \hline
    \end{tabular}}
    \caption{
    %An interpretation translation with a distinguishable style delivers the source message as faithful as its corresponding offline translation.
    Translation and interpretation differ in 
    %possess different 
    style while conveying the same source information.
    }
    \vspace{-2.5mm}
    \label{tab:intro_example}
\end{table}

==> tables/strategy.tex <==
\begin{table*}
\centering
\small
  \scalebox{0.85}
  {
  \begin{tabular}{l|p{5cm}|p{5cm}|p{5cm}}
    \toprule
    \textbf{Strategy} & \textbf{Source} & \textbf{Interpreted Text}  & \textbf{Translated Text}  \\
    \midrule
    Segment \textcolor{orange}{$\vert\vert\vert$} & Man kann darüber streiten, ob die Modellpolitik der europäischen Hersteller, insbesondere der deutschen, verantwortlich war für die Krise, die wir jetzt haben. & You can argue whether the model policy of the European manufacturers in particular. \textcolor{orange}{$\vert\vert\vert$} The German one was responsibility for the crisis that we have. & People can argue about whether the choice of models produced by European manufacturers, especially the German manufacturers, was responsible for the crisis we are now in. \\
    \textcolor{DarkBlue}{Generalize} & Herr Präsident, meine Damen und Herren! Sicherheit ist ein hohes Gut. & President ladies and gentlemen safety is \textcolor{DarkBlue}{very important}. & Mr President, ladies and gentlemen, safety is \textcolor{DarkBlue}{a sacred thing}. \\
    \greenuline{Summarize}, \textcolor{DarkGreen}{(Omit)} & Ich werde an diesem Punkt darauf verzichten, einen Kommentar zur Ernsthaftigkeit dieser Argumentationsweise abzugeben.& I'm not going to comment on \greenuline{that agreement}. & \textcolor{DarkGreen}{(At this point,)} I will refrain from commenting on \greenuline{the seriousness of this line of argument}.  \\
    \redwave{Passive} & Die Frage der Exterritorialität wäre auch zu lösen. & The extraterritorial question also \redwave{needs to be resolved}. & We \redwave{must also resolve} the question of extraterritoriality. \\
    \bottomrule
  \end{tabular}
  }
  \caption{Examples of strategies exhibited in interpreted texts, in comparison with corresponding translated texts.}
  \label{tab:strategies}
\end{table*}

